JArena: Partitioned Shared Memory for NUMA-awareness in Multi-threaded Scientific Applications

The distributed shared memory (DSM) architecture is widely used in today's computer design to mitigate the ever-widening processing-memory gap, and inevitably exhibits non-uniform memory access (NUMA) to shared-memory parallel applications. Failure to achieve full NUMA-awareness can significantly downgrade application performance, especially on today's manycore platforms with tens to hundreds of cores. Yet traditional approaches such as first-touch and memory policy fail short in either false page-sharing, fragmentation, or ease-of-use. In this paper, we propose a partitioned shared memory approach which allows multi-threaded applications to achieve full NUMA-awareness with only minor code changes and develop a companying NUMA-aware heap manager which eliminates false page-sharing and minimizes fragmentation. Experiments on a 256-core cc-NUMA computing node show that the proposed approach achieves true NUMA-awareness and improves the performance of typical multi-threaded scientific applications up to 4.3 folds with the increased use of cores.

==> Makefile <==
#
# Makefile for latex documents
#

# Description of the document structure
INDEX_DOC = main.tex
SECT_DOCS = introduction.tex  \
						background-and-motivation.tex \
						partitioned-shared-memory.tex \
						jarena-algorithms.tex \
						experimental-evaluation.tex \
						related-works.tex \
						conclusion-and-outlook.tex

BIBTEX_DOC = references.bib
#OUTPUT_DOC := $(subst .tex,.pdf,$(INDEX_DOC))
OUTPUT_DOC = paper.pdf
STYLE_DOCS = llncs.cls llncsconf.sty splncs04.bst

# Configuration of latex toolchain
PDFLATEX := pdflatex # could be pdflatex or xelatex
BIBTEX := bibtex

.PHONY: clean view
all: $(OUTPUT_DOC)

INDEX_STEM = $(subst .tex,,$(INDEX_DOC))
$(OUTPUT_DOC): $(INDEX_DOC) $(SECT_DOCS) $(BIBTEX_DOC) $(STYLE_DOCS)
	$(PDFLATEX) $(INDEX_STEM)
	- $(BIBTEX) $(INDEX_STEM)
	$(PDFLATEX) $(INDEX_STEM)
	$(PDFLATEX) $(INDEX_STEM)
	mv $(INDEX_STEM).pdf $(OUTPUT_DOC)

VIEWER := xdg-open
UNAME_S := $(shell uname -s)
ifeq ($(UNAME_S),Linux)
	VIEWER = xdg-open
endif
ifeq ($(UNAME_S),Darwin)
	VIEWER = open
endif
view: $(OUTPUT_DOC)
	$(VIEWER) $^

INTERN_POSTFIXES = .aux .bbl .blg .log .out .upa .upb
INTERN_DOCS = $(foreach p,$(INTERN_POSTFIXES),$(INDEX_STEM)$(p))
INTERN_DOCS += *synctex* *.bak*
clean:
	rm -f $(INTERN_DOCS) $(OUTPUT_DOC)

